A G\"odel Modal Logic Over Witnessed Models

We introduce GW, a G\"odel modal logic based on Kripke models in which the value of each modal formula is witnessed by an accessible world. This witnessed semantics eliminates the limit-based phenomena that preclude the finite model property in the usual Kripke semantics for G\"odel modal logics, thereby yielding a more constructive semantic framework. We present a sound and complete refutation calculus for GW and design a terminating backward proof-search procedure with countermodel generation. As a direct consequence of this procedure, GW enjoys the finite model property.

==> eptcsdata.tex <==
\providecommand{\firstpage}{355}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.20}{10.4204/EPTCS.447.20}}

